StuffNet: Using 'Stuff' to Improve Object Detection

We propose a Convolutional Neural Network (CNN) based algorithm - StuffNet - for object detection. In addition to the standard convolutional features trained for region proposal and object detection [31], StuffNet uses convolutional features trained for segmentation of objects and 'stuff' (amorphous categories such as ground and water). Through experiments on Pascal VOC 2010, we show the importance of features learnt from stuff segmentation for improving object detection performance. StuffNet improves performance from 18.8% mAP to 23.9% mAP for small objects. We also devise a method to train StuffNet on datasets that do not have stuff segmentation labels. Through experiments on Pascal VOC 2007 and 2012, we demonstrate the effectiveness of this method and show that StuffNet also significantly improves object detection performance on such datasets.

==> sections/discussion.tex <==
\section{Discussion} \label{sec:5}
Conclusion

==> sections/figures.tex <==
\begin{figure*}[h!]
  \centering
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/0_f}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/0_s}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/2_f}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/2_s}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/6_f}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/6_s}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/5_f}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/5_s}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/4_f}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/4_s}
  \end{subfigure}  
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/1_f}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/1_s}
  \end{subfigure}
\caption{Pairs of Faster R-CNN (left) vs. \texttt{StuffNet-30} (right) detections on sample images from the Pascal VOC 2010 \texttt{test}. Both models have been trained on Pascal VOC 2010 \texttt{trainval}}
\label{fig:4}
\end{figure*}
\begin{figure*}[h!]
  \centering
	\begin{subfigure}[b]{0.22\textwidth}
    	\includegraphics[width=\textwidth]{images/seg_in0.jpg}
        \includegraphics[width=\textwidth]{images/seg_in1.jpg}
        \includegraphics[width=\textwidth]{images/seg_in2.jpg}
        \caption{Image}
	\end{subfigure}
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{images/seg_out0_2010_10.jpg}
        \includegraphics[width=\textwidth]{images/seg_out1_2010_10.jpg}
        \includegraphics[width=\textwidth]{images/seg_out2_2010_10.jpg}
        \caption{StuffNet-10}
	\end{subfigure}
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{images/seg_out0_2010_30.jpg}
        \includegraphics[width=\textwidth]{images/seg_out1_2010_30.jpg}
        \includegraphics[width=\textwidth]{images/seg_out2_2010_30.jpg}
        \caption{StuffNet-30}
        \label{fig:5c}
	\end{subfigure}
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{images/seg_out0_2012_30.jpg}
        \includegraphics[width=\textwidth]{images/seg_out1_2012_30.jpg}
        \includegraphics[width=\textwidth]{images/seg_out2_2012_30.jpg}
        \caption{StuffNet-30}
        \label{fig:5d}
	\end{subfigure}
    \begin{subfigure}[b]{0.10\textwidth}
    	\includegraphics[width=\textwidth, height=0.395\textheight]{images/legend}
        \caption{legend}
        \label{fig:5e}
     \end{subfigure}
\caption{StuffNet segmentation qualitative results on images from the MS COCO dataset. Models (b) and (c) were trained on Pascal VOC 2010 \texttt{trainval}, while (d) was trained on Pascal VOC 2012 \texttt{trainval} using feature constraining.}
\label{fig:5}
\end{figure*}
%\begin{figure*}[h!]
%  \centering
%	\begin{subfigure}[b]{0.3\textwidth}
%    	\includegraphics[width=\textwidth]{images/supp/2_f}
%    \includegraphics[width=\textwidth]{images/supp/1_f}
%    \includegraphics[width=\textwidth]{images/supp/0_f}
%    \includegraphics[width=\textwidth]{images/supp/3_f}
%    \includegraphics[width=\textwidth]{images/supp/10_f}
%    \includegraphics[width=\textwidth]{images/supp/12_f}
%    \caption{Faster R-CNN}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.3\textwidth}
%    	\includegraphics[width=\textwidth]{images/supp/2_s}
%    \includegraphics[width=\textwidth]{images/supp/1_s}
%    \includegraphics[width=\textwidth]{images/supp/0_s}
%    \includegraphics[width=\textwidth]{images/supp/3_s}
%    \includegraphics[width=\textwidth]{images/supp/10_s}
%    \includegraphics[width=\textwidth]{images/supp/12_s}
%    \caption{\texttt{StuffNet-30}}
%	\end{subfigure}	
%	\begin{subfigure}[b]{0.3\textwidth}
%    	\includegraphics[width=\textwidth]{images/supp/2_seg}
%    \includegraphics[width=\textwidth]{images/supp/1_seg}
%    \includegraphics[width=\textwidth]{images/supp/0_seg}
%    \includegraphics[width=\textwidth]{images/supp/3_seg}
%    \includegraphics[width=\textwidth]{images/supp/10_seg}
%    \includegraphics[width=\textwidth]{images/supp/12_seg}
%    \caption{~\texttt{StuffNet-30}}
%	\end{subfigure}	
%	\begin{subfigure}[b]{0.08\textwidth}
%			\includegraphics[width=\textwidth]{images/supp/legend}
%			\caption{Legend}
%	\end{subfigure}	
%\caption{\texttt{StuffNet-30} detection and segmentation qualitative results on images from the MS COCO dataset. The model was trained on Pascal VOC 2010 \texttt{trainval}. We also show Faster R-CNN detections in the first column for comparison. \texttt{StuffNet-30} performs particularly well in detecting small objects.}
%\label{fig:6}
%\end{figure*}

==> sections/training.tex <==
\section{Training} \label{sec:3}
In this section we describe the procedure used for training the two branches and the fusion module described in Section~\ref{sec:2}. The two convolution layer groups common to both the branches are initialized from the publicly available VGG 16 layer model. We set the learning rates of these layers to 0 while training, so that their weights do not change. This is because the low level features learnt by these two groups of convolution layers are useful for both the object detection as well as semantic segmentation tasks.

\subsection{Stuff segmentation branch} \label{sec:3.1}
We first train the stuff semantic segmentation network to perform semantic segmentation. Then we set the learning rates of the layers in the stuff semantic segmentation branch (\texttt{conv3-seg} - \texttt{conv5-seg}, \texttt{fc6-seg} and \texttt{fc7-seg}) to 0 and use them as a feature extractor as described in Section~\ref{sec:2.2} to train the object detection branch and the fusion module in  an end-to-end fashion. This strategy enables us to learn the stuff segmentation features from datasets that label stuff (e.g. Pascal Context~\cite{mottaghi} and NYU Depth V2~\cite{nyu_dv2}) and reuse them for other datasets where stuff labels are not available (e.g. MS COCO~\cite{ms_coco}). This makes the assumption that the distribution of mean-subtracted stuff category pixels remains the same across datasets. We have qualitatively concluded that this assumption is valid, because stuff is mostly homogeneous in appearance. For example, Figure~\ref{fig:3} shows the output of the stuff segmentation network on an image taken from the MS COCO dataset. The network was trained by using a combination of images from the Pascal Context and NYU Depth V2 datasets.

\begin{figure}
\centering
\subfloat[][image]{\includegraphics[width=0.47\textwidth]{images/seg_im}}
\subfloat[][segmentation]{\includegraphics[width=0.47\textwidth]{images/seg_seg}}
\caption{Stuff semantic segmentation of an image from the MS COCO dataset, produced by the network trained on the Pascal Context and NYU Depth v2 datasets. \textit{green}: tree, \textit{gray}: ground, \textit{blue}: sky, \textit{purple}: building, \textit{black}: background}
\label{fig:3}
\end{figure}

We merge training data from the Pascal Context and NYU Depth V2 datasets and pick the 10 most prominent stuff categories: \texttt{wall, table, floor, water, tree, sky, road, ground, building} and \texttt{shelves}. We merge the \texttt{sidewalk} and \texttt{runway} categories into \texttt{road}, and \texttt{grass, platform, sand, snow} into the \texttt{ground} category for the Pascal Context dataset. For the NYU Depth V2 dataset, we merge \texttt{door} and \texttt{whiteboard} into \texttt{wall}, and \texttt{cabinet} and \texttt{bookshelves} into the \texttt{shelves} category. After a 80\%-20\% train-test split, we have 8611 training images and 2152 testing images. We train the network to minimize a softmax loss as described in Section~\ref{sec:2.2} using stochastic gradient descent (SGD) for 30K iterations. The learning rate starts at 1e-3 and drops by a factor of 10 every 10K iterations. Momentum is set to 0.9 and weight decay to 0.0005. Our stuff semantic segmentation network gives 51.72\% mean pixel-wise accuracy over our testing dataset. It is important to note that since we use the \texttt{fc7-seg} features from the stuff semantic segmentation branch, the labelling accuracy of the branch only serves as a rough indicator of the effectiveness of the features learnt by the convolutional layers.

\subsection{Object detection branch and fusion module} \label{sec:3.2}
The convolution layers (\texttt{conv3} - \texttt{conv5}) and fully connected layers (\texttt{fc6} and \texttt{fc7}) in this branch are also initialized from the publicly released VGG 16 layer model. The layers in the stuff segmentation branch (\texttt{conv3-seg} - \texttt{conv5-seg}, \texttt{fc6-seg} and \texttt{fc7-seg}) are initialized from the already trained stuff segmentation network. All the other layers (\texttt{bbox-pred, fc7-seg-project} and \texttt{fc-fuse}) have their weights initialized randomly from a zero mean, 0.01 variance Gaussian, and their biases initialized to zero.

The learning rates for the two common convolutional layer groups (\texttt{conv1} and \texttt{conv2}) and layers in the stuff segmentation branch (\texttt{conv3-seg} - \texttt{conv5-seg}, \texttt{fc6-seg} and \texttt{fc7-seg}) are set to 0 while training the object detection branch. We use the values of training hyperparameters mentioned in~\cite{fast_rcnn}. The batch size needs to be reduced from 2 to 1, so that both branches of the network can be loaded into the GPU. We double the number of SGD iterations to compensate for this.
